Asymptotic Experiments with Data Structures: Bipartite Graph Matchings and Covers

We consider instances of bipartite graphs and a number of asymptotic performance experiments in three projects: (1) top movie lists, given databases of movies and viewers, (2) maximum matchings, and (3) minimum set covers. Experiments are designed to measure the asymptotic runtime performance of abstract data types (ADTs) in three programming languages: Java, R, and C++. The outcomes of these experiments may be surprising. In project (1), the best ADT in R consistently outperforms all ADTs in public domain Java libraries, including the library from Google. The largest movie list has $2^{20}$ titles. In project (2), the Ford-Fulkerson algorithm implementation in R significantly outperforms Java. The hardest instance has 88452 rows and 729 columns. In project (3), a stochastic version of a greedy algorithm in R can significantly outperform a state-of-the-art stochastic solver in C++ on instances with $num\_rows \ge 300$ and $num\_columns \ge 3000$.

==> _preambles/preamble_elsarticle.tex <==

\usepackage{lineno,hyperref}
\usepackage{doi}
\modulolinenumbers[5]
\usepackage{framed}
\newcommand{\thedate}{\today}
\journal{}
% Prepripnt is removed
\makeatletter
\def\ps@pprintTitle{%
 \let\@oddhead\@empty
 \let\@evenhead\@empty

%% CUSTOMIZE THIS FOOTNOTE HERE111 %%
 \def\@oddfoot{
\begin{footnotesize}
\begin{tabular}{p{0.85\textwidth}}
 ~ \\
\hline
 \multicolumn{1}{|p{0.85\textwidth}|}{
 \footnotesize   \mtext{This manuscript, created on \thedate, is being drafted for posting on the server at \url{http://arxiv.org/} and as a journal submission for a peer review. Authors welcome comments and suggestions from readers at all times.} 
 } \\
 %Currently, the manuscript is also undergoing anonymous peer reviews.} \\
% 
% \footnotesize This version, created on \@date, is an electronic reprint of the original article published in the Applied Soft Computing Journal, 2017, Vol. 56, pp. 262--285,
% \href{http://dx.doi.org/10.1016/j.asoc.2017.02.024}{doi:10.1016/j.asoc.2017.02.024}. This reprint differs from the original in pagination and typographic detail.} \\
 \hline
\end{tabular}
\end{footnotesize}
 }%
 
 
 \let\@evenfoot\@oddfoot
 }
\makeatother


%%%%%%%%%%%%%%%%%%%%%%%
%% Elsevier bibliography styles
%%%%%%%%%%%%%%%%%%%%%%%
%% To change the style, put a % in front of the second line of the current style and
%% remove the % from the second line of the style you would like to use.
%%%%%%%%%%%%%%%%%%%%%%%

%% Numbered
%\bibliographystyle{model1-num-names}

%% Numbered without titles
%\bibliographystyle{model1a-num-names}

%% Harvard
%\bibliographystyle{model2-names.bst}\biboptions{authoryear}

%% Vancouver numbered
%\usepackage{numcompress}\bibliographystyle{model3-num-names}

%% Vancouver name/year
%\usepackage{numcompress}\bibliographystyle{model4-names}\biboptions{authoryear}

%% APA style
%\bibliographystyle{model5-names}\biboptions{authoryear}

%% AMA style
%\usepackage{numcompress}\bibliographystyle{model6-num-names}

%% `Elsevier LaTeX' style
\bibliographystyle{elsarticle-num}
%%%%%%%%%%%%%%%%%%%%%%%

% From authors
\usepackage{algorithmic}
\usepackage{amssymb}
\usepackage{color}
\usepackage{multirow}
% \newcommand{\rework}[1]{\textcolor{red}{#1}}

\usepackage{hyperref}
\hypersetup{colorlinks,urlcolor=blue}


\usepackage{lipsum} % Package to generate dummy text throughout this template
\usepackage{subfig}
\usepackage{graphicx}


